M. Kontsevich's graph complex and the Grothendieck-Teichmueller Lie algebra

We show that the zeroth cohomology of M. Kontsevich's graph complex is isomorphic to the Grothendieck-Teichmueller Lie algebra grt_1. The map is explicitly described. This result has applications to deformation quantization and Duflo theory. We also compute the homotopy derivations of the Gerstenhaber operad. They are parameterized by grt_1, up to one class (or two, depending on the definitions). More generally, the homotopy derivations of the (non-unital) E_n operads may be expressed through the cohomology of a suitable graph complex. Our methods also give a second proof of a result of H. Furusho, stating that the pentagon equation for grt_1-elements implies the hexagon equation.

==> alternative_proof.tex <==
% don't forget this.... maybe useful for something

%\begin{rem}
%$\Def(\hoe_n\to \fGraphs_{n,c}^\whl)_\conn$ may be equipped with a filtration by the number of clusters of size one and valence one (using the terminology from Appendix \ref{sec:defengra}). By a combinatorial argument, one may then compute the first convergent of the associated spectral sequence and find that it is isomorphic to $\fGC_{n,\conn}[-1]\oplus \GF[-1]$. This can be made into a quick proof of Theorem \ref{thm:GCdef}. We will however follow a different route below. 
%\end{rem}

==> appdd.tex <==
\section{Application: Checking the Deligne-Drinfeld conjecture in low orders}
\label{sec:appdd}
Consider the conjectural generators $\sigma_j$ (for odd $j\geq 3$) of $\grt$. It is clear that the set of $\sigma_j$'s is linearly independent because of the grading on $\grt$ by ``number of $t_{ij}$'s''. Next consider the commutators 
\[
 \sigma_{ij} = \co{\sigma_i}{\sigma_j}.
\]
Fix $N:= i+j$. Then the $\sigma_{ij}$ span a vector space 
\[
V_N := \vsspan \{\sigma_{ij} \mid i>j\geq 3, i,j \text{ odd}, i+j=N \}.
\]
The Deligne-Drinfeld conjecture asserts that the $\sigma_{ij}$ for $i>j\geq 3$ are linearly independent and hence conjecturally
\[
 \dim V_N = \lfloor \frac{1}{4}N-1 \rfloor \quad\quad\quad \text{(conjecture)}.
\]
The main result of this section is the following lower bound.
\begin{prop}
\label{prop:VNlowerbound}
Let $N$ be an even positive integer. The space $V_N\subset \grt$ spanned by $\{\sigma_{ij} \mid i>j\geq 3, i,j \text{ odd}, i+j=N \}$ is at least $\lceil \frac{1}{6}N -1\rceil$-dimensional.
\end{prop}

The proof proceeds by explicitly constructing a series of homology classes in the dual of the graph complex.
The graph complex $\GC$ splits into a direct sum of finite dimensional sub-complexes
\[
 \GC = \oplus_\alpha \GC^{(\alpha)}
\]
as discussed in Appendix \ref{sec:specs}. We define the graded dual of $\GC$ as the complexes
\[
 \GC^* :=  \oplus_\alpha (\GC^{(\alpha)})^*.
\]
%\begin{rem}
 Recall that elements of $\GC$ are linear combinations of graphs (with numbered vertices), invariant under permutations of the vertex labels. Similarly, elements of $\GC^*$ should be thought of as linear cominations of graphs with numbered vertices, modulo permutations of the vertex labels. It is clear that there is a natural pairing 
\[
 \skp{\cdot}{\cdot} \colon \GC^* \times \GC \to \R.
\]
From this and the dg Lie algebra structure on $\GC$, one obtains a dg Lie coalgebra structure on $\GC^*$.
Concretely, the differential on $\GC^*$ is given by edge contraction.
%\end{rem}

It is possible to compute a series of degree zero homology classes of $\GC^*$. By using the pairing $\GC^* \times \GC\to \R$ one can extract from this series linear independence properties of classes in $H^0(\GC)\cong \grt$.

Let us start with the simplest (and admittedly trivial) example. Let $\sigma_{j}$, for odd $j\geq 3$, by abuse of notation also denote representatives in $\GC$ of the cohomology classes corresponding to the conjectural generators of $\grt$, see Section \ref{sec:explgenerators} for details. By Proposition \ref{prop:sigmawheel} $\sigma_{j}$ contains a term corresponding to a wheel-graph with $j$ spokes as in Figure \ref{fig:wheelgraphs}. Since the wheel graph is not closed for $j>3$, $\sigma_{j}$ will in general also contain other terms. However, dually in $\GC^*$, all wheel graphs are closed and hence define homology classes. Let us denote by $s_{j}\in \GC^*$, for odd $j\geq 3$, the wheel graph with $j$ spokes. It is a piori not clear that the $s_{j}$ represent nontrivial homology classes. However, if we normalize correctly, we know that 
\[
 \skp{s_{i}}{\sigma_{j}} = \delta_{ij}.
\]
From this statement one can immediately conclude that
\begin{enumerate}
 \item The homology classes $\{[s_{j}] \mid j=3,5,\dots \}$ are linearly independent.
 \item The cohomology classes $\{[\sigma_{j}] \mid j=3,5,\dots \}$ are linearly independent.
\end{enumerate}

Let us go further and look at the first commutators $\sigma_{ij} := \co{\sigma_i}{\sigma_j} = - \sigma_{ji}$.\footnote{Here again we abuse earlier notation and understand $\sigma_{ij}$ as cocycles in the graph complex, rather than elements of $\grt$.} Now suppose that the we had cycles $s_{ij}=-s_{ji}\in \GC^*$ such that
\[
 \skp{s_{ij}}{\sigma_{kl}} = \delta_{ik}\delta_{jl} - \delta_{il}\delta_{jk}.
\]
Then we could conclude as above that the cohomology classes $[\sigma_{ij}]\in H^0(\GC)$ ($i,j=3,5,\dots $ and $i<j$) and the homology classes $[\sigma_{ij}]\in H^0(\GC^*)$ ($i,j=3,5,\dots $ and $i<j$) both form linearly independent families.
Unfortunately, I cannot write down all the $s_{ij}$ or arbitrary odd $i$ and $j$. However, I can write down formulas for a smaller series of homology classes $t_{pq}$, where $p>q>0$ and $q$ is even. Each $t_{pq}$ will be a linear combination of graphs with $2p+q+1$ vertices. Deferring the definition, the $t_{pq}$ will satisfy the following properties.
\begin{prop}
\label{prop:tpq}
 \begin{enumerate}
  \item \label{proptpqliit} The homology classes $\{ [t_{pq}]\mid p>q>0, q \text{ even} \}$, are linearly independent.
  \item \label{proptpqVit} Let 
\[
 \iota \colon V:=\vsspan \{ [\sigma_{ij}] \mid i> j\geq 3, i,j \text{ odd} \} \to H^0(\GC)
\]
be the inclusion.
Then the homology classes $\{ \iota^*[t_{pq}]\mid p>q>0, q \text{even} \}$, are still linearly independent.
  \item \label{proptpqSit} Let $p,q,i,j$ be integers such that $p>q>0$, $q$ is even, $i>j\geq 3$ and $i$ and $j$ are odd. Then
\[
\skp{t_{pq}}{\sigma_{ij}} = 
\begin{cases}
\pm z_{i-p-1}(p-q, j-1)  &\text{if $i+j=2p+q$, and $i>p\geq j$} \\
0 &\text{otherwise} 
\end{cases}
\]
where
\begin{equation}
\label{equ:zawdef}
 z_k(\alpha,\beta) = { k \choose \frac{k+\alpha-\beta}{2} } - { k \choose \frac{k+\alpha+\beta}{2} }
\end{equation}
is the number of zero avoiding $k$-step walks from $\alpha$ to $\beta$ (see the remark below).
\item The $t_{pq}\in \GC^*$ vanish on all triple (or higher) commutators in $\GC$, i.e.
\[
\skp{t_{pq}}{\co{\co{x}{y}}{z}} = 0 
\]
for all $x,y,z \in \GC$ and for all integers $p,q$ such that $p>q>0, q \text{even}$.
\end{enumerate}
\end{prop}
\begin{rem}
 Let $\alpha, \beta$ be positive integers, and let $k$ be an integer such that $k\geq |\alpha-\beta|$ and $k\equiv \alpha-\beta \mod 2$. A $k$-step walk from $\alpha$ to $\beta$ is a $k$-tuple $(c_1,\dots, c_k)$ with $c_1,\dots, c_k\in \{\pm 1\}$ such that 
$\beta = \alpha + \sum_{i=1}^k c_i$. The walk is called zero-avoiding if the partial sums $\alpha + \sum_{i=1}^jc_i$ are all positive for $j=1,\dots, k$. 
\end{rem}

\begin{proof}[Proof of Proposition \ref{prop:VNlowerbound}]
 Consider statement \ref{proptpqVit} of the proposition above. It is clear that the space $V$ therein decomposes into a direct sum of spaces $V_N$. Concretely, $V_N$ is the subspace of (co)homology classes representable by linear combinations of graphs with $N+1$ vertices. On the dual side, the $t_{pq}$ are linear combinations of graphs with $2p+q+1$ vertices. Since the pairing (of course) respects the number of vertices, the restrictions of $\iota^*[t_{pq}]$ to $V_N$, with $2p+q=N$, are still linearly independent. A small calculation shows that there are $\lceil \frac{1}{6}N -1\rceil$ allowed combinations of $p,q$ (i.e., $p>q>0$ and $2p+q=N$), and hence $V_N$ must have at least that dimension.
\end{proof}

\begin{rem}
The Deligne-Drinfeld conjecture asserts that $\dim V_N = \lfloor \frac{1}{4}N-1 \rfloor$. Hence asymptotically as $N\to\infty$, one sees that the homology classes $[t_{pq}]$ account for $\frac{2}{3}$ of the expected homology. I tried for some time to find closed formulas for the missing third as well, but without success. Computer experiments indicate that formulas for the missing third, at least if expressed using graphs, are significantly more complicated than the formulas for the $t_{pq}$. This is very mysterious to me. What distinguishes the elements of $\grt^*$ for which there are relative simple formulas from those for which there are none? Is there some underlying reason, or some other way to characterize those elements?
\end{rem}

\begin{figure}
 \centering
\input fig_thetagdef.tex
\caption{\label{fig:thetaGdef} The top left graph is the graph $\Theta(5,4,2)$. On the top right the general scheme for generating the graphs $\Theta(p,q,r)$ is depicted. The ``upper arc'' should consist of $p$ edges, the middle arc of $q$ and the bottom arc of $r$ edges. Concretely, it means that the upper ``$\dots$'' represent $p-5$ vertices, the middle ``$\dots$'' $q-3$ and the lower ``$\dots$'' $r-5$ vertices. The bottom graph in this Figure is the graph $G(7,5)$. We have not drawn the general scheme for the $G(p,q)$ as it should be clear. }
\end{figure}

Let us now define the $t_{pq}$ and give a proof of the above proposition.
We will need two different kinds of graphs, denoted $\Theta(p,q,r)$, depending on 3 positive integers $p,q,r$ and $G(p,q)$, depending on two positive integers $p,q$. Instead of giving a formal definition, we refer to Figure \ref{fig:thetaGdef}, from which it should be clear.
We will consider $\Theta(p,q,r)$ and $G(p,q)$ as elements of $\GC^*$. Then the following relations hold by symmetry:
\begin{align*}
\Theta(p,q,r) &= \Theta(q,r,p) = -\Theta(q,p,r) \\
G(p,q) &= -(-1)^{p}G(p,q) = -(-1)^{q}G(p,q)
\end{align*}

In particular, for example $\Theta(p,p,r)=0$ for all $p,r$ and $G(p,q)=0$ if $p$ or $q$ is even.
Now we are ready to write down the formula for $t_{pq}$.
\begin{multline*}
 t_{pq} = \sum_{ \substack{ 0<i\leq p \\ 0<j \leq q \\ i> j} } (-1)^{p+q-i-j} z_{p+q-i-j}(p-q,i-j) \Theta(2p+q+1 -i-j ,i,j)
\\
+ \sum_{0<i\leq p} (-1)^{p+q-i} z_{p+q-i-1}(p-q,i-1) G(2p+q-i,i) 
\end{multline*}

where the $z_{\dots}(\dots)$ denotes again the number of zero avoiding walks as in equation \eqref{equ:zawdef}. 
Note that by the symmetries of $G(p,q)$, the terms in the second sum for even $i$ are all zero. We merely keep them for simplicity of notation,

To see that the $t_{pq}$ thus defined are actually closed, we need to compute the differentials in $\GC^*$ of $\Theta(p,q,r)$ and $G(p,q)$. If one defines the signs correctly, one finds that 
\begin{align*}
\delta\Theta(p,q,r) &= \hat \Theta(p-1,q,r) + \hat \Theta(p,q-1,r) + \hat \Theta(p,q,r-1) \\
\delta G(p,q) &= \hat \Theta(p,q,0)
\end{align*}
where the graphs $\hat \Theta(p,q,r)$ are defined graphically in Figure \ref{fig:hatthetadef}.
They satisfy the following symmetry properties.
\begin{align*}
 \hat \Theta(p,q,r) &=  \hat \Theta(q,r,p) =  -\hat \Theta(q,p,r) \\
 \hat \Theta(p,q,r) &= (-1)^{p+q+r} \hat \Theta(p,q,r) \\
 \hat \Theta(p,q,0) &= -(-1)^{p} \hat \Theta(p,q,0)
\end{align*}

\begin{figure}
 \centering
\input fig_hatthetadef.tex
\caption{\label{fig:hatthetadef} On the left the graph $\hat \Theta(p,q,r)$ is depicted. Note that the difference to $\Theta(p,q,r)$ is merely one edge. However, this edge creates a new symmetry by reflection around a vertical line. Here we allow also that one of the parameters is 0. For example, the graph $\hat \Theta(5,3,0)$ is shown on the right.}
\end{figure}

Now compute:
\begin{align*}
  \delta t_{pq} 
&=
\sum_{ \substack{ 0<i\leq p \\ 0<j \leq q \\ i> j} } (-1)^{p+q-i-j} z_{p+q-i-j}(p-q,i-j) 
\\ &\quad\quad
\left( \hat \Theta(2p+q -i-j ,i,j) + \hat \Theta(2p+q+1 -i-j ,i-1,j) + \hat \Theta(2p+q+1 -i-j ,i,j-1)\right)
\\ &\quad\quad
+ \sum_{0<i\leq p} (-1)^{p+q-i} z_{p+q-i-1}(p-q,i-1) \hat \Theta(2p+q-i,i,0).
\end{align*}

Let us collect the coefficient in front of $\hat \Theta(2p+q -i-j ,i,j)$ (for $2p+q -i-j>i>j>0$):
\begin{multline*}
 (-1)^{p+q-i-j} z_{p+q-i-j}(p-q,i-j) 
+ \delta_{i<p} (-1)^{p+q-i-1-j} z_{p+q-i-1-j}(p-q,i+1-j) 
\\ + \delta_{j<q} \delta_{j+1<i} (-1)^{p+q-i-j-1} z_{p+q-i-j-1}(p-q,i-j-1)
\\
=
\pm
\left( 
z_{p+q-i-j}(p-q,i-j) -\delta_{i<p} z_{p+q-i-1-j}(p-q,i+1-j)  \right.
\\
\left. - \delta_{j<q}\delta_{j+1<i} z_{p+q-i-j-1}(p-q,i-j-1)
\right) 
\end{multline*}

Here $\delta_{(\dots)}$ is defined to be $1$ if the condition $(\dots)$ is true and $0$ otherwise.
The term on the right hand side is zero by the following equation for zero-avoiding walks.\footnote{The equation is obtained by splitting each walk with $k+1$ steps into one with $k$ steps, plus a last step which can either go up (second term) or down (first term). The $\delta_{(\dots)}$ in the equation may be omitted if one defines $z_k(\alpha,\beta)=0$ for ``bad'' values of the parameters.}
\[
 z_{k+1}(\alpha, \beta) = 
\delta_{k\geq \beta+1-\alpha} z_{k+1}(\alpha, \beta+1)
 +
\delta_{\beta>1}
\delta_{k\geq \alpha+1-\beta}
z_{k+1}(\alpha, \beta-1).
\]

We have not yet considered here the $\hat \Theta(2p+q-i,i,0)$, i.e., those $\hat \Theta$'s whose last argument is $0$. Those terms are contributed from the second sum, and from the first if $j=1$. The total coefficient is
\[
 (-1)^{p+q-i-1} z_{p+q-i-1}(p-q,i-1)
+
 (-1)^{p+q-i} z_{p+q-i-1}(p-q,i-1)
=0.
\]

Hence we have seen that indeed the $t_{pq}$ are cocycles.

\begin{proof}[Proof of Proposition \ref{prop:tpq}]
The space $\GC^*$ carries a dg Lie coalgebra structure dual to the dg Lie algebra structure on $\GC$. 
Concretely, the cobracket of a graph $\Gamma$ is computed by identifying complete subgraphs all of whose vertices are at least trivalent and contracting them:
\[
 \Delta \Gamma = \sum_{\Gamma'\subset \Gamma} \Gamma / \Gamma' \wedge \Gamma' \cdot (\text{prefactor depending on conventions}).
\]
Here $\Gamma / \Gamma'$ means the graph obtained from $\Gamma$ by contracting $\Gamma'$ to one vertex.
For example, one can easily see that the cobracket of any wheel graph (see Figure \ref{fig:wheelgraphs}) is zero. Similarly, the cobracket of the graphs $\Theta(p,q,r)$ is zero. The cobracket of the graphs $G(p,q)$ on the other hand is a product of a wheel graph with $p$ spokes and one with $q$ spokes. Hence the double cobracket of any $t_{pq}$ is zero, which is the last assertion of the proposition.
Also, knowing the cobracket of $t_{pq}$ one computes (using Sweedler notation)
\[
\skp{t_{pq}}{\sigma_{ij}} = \skp{t_{pq}}{\co{\sigma_i}{\sigma_j}}
=\sum \skp{t_{pq}'}{\sigma_i} \skp{t_{pq}''}{\sigma_j}
= (\text{coefficient of $G(i,j)$})
\]
Hence one obtains assertion \ref{proptpqSit} of the proposition.

Finally we want to prove assertion \ref{proptpqVit} from which assertion \ref{proptpqliit} obviously follows. Without loss of generality we fix the number of vertices to be $N+1$. So assume that there is some linear combination $t$ of the $t_{pq}$ vanishing on all $\sigma_{ij}$. This means that $t$ has the form
\[
t = \sum_{\substack{ i> j > 1 \\ N > 2i + j }}  (-1)^{i+j} c_{ij} \Theta(N+1-i-j, i,j)                                                                                                                                                                                                                                               \]
 for some yet unknown constants $c_{ij}$. Note that there are no $G(p,q)$-terms by the condition that $t$ vanishes on all $\sigma_{ij}$ and the first part of this proof. We also know that $t$ is a cycle, i.e., $\delta t=0$. In terms of the $c_{ij}$ this amounts to the following system of equations
\begin{align*}
c_{i1} &= 0 &\text{for $i$ odd} \\
c_{ij} &= \delta_{N>2i+j+1} c_{i+1,j} + \delta_{i>j+1}c_{i,j+1}. &
\end{align*}
The derivation of these equations proceeds as in the calculation of $\delta t_{pq}=0$ above.
These equations can be solved by an induction on $k=i+j$. The result is that $c_{ij}=0$ for all $i,j$. This is not obvious, but a standard exercise, so we omit the calculation. Hence we know that $t=0$. On the other hand, $t$ was a linear combination of $t_{pq}$'s, with fixed $N=2p+q$. But the graph $\Theta(p+1,p,q)$ occurs only in $t_{pq}$ and hence the linear combination must be trivial. 
\end{proof}

\begin{rem}
It also follows from Proposition \ref{prop:tpq} that $[\sigma_{ij}]\neq 0$ for all odd $i\neq j$. This is a well-known result. 
\end{rem}



==> appduflo.tex <==
\section{Application: Duflo formulas}


==> appgrt.tex <==
\section{The Grothendieck-Teichm\"uller Lie algebra}


==> ginfty.tex <==
\section{$G_\infty$ morphism and relation to Tamarkin's quantization}
In this section we show how to canonically convert our $KS_\infty$ morphism and prove Proposition \ref{prop:ginfty}. First construct a map $G_\infty \to \KS_\infty$ by lifting up to homotopy:
\[
 \begin{tikzpicture}
  \matrix(m)[diagram]{ &  & \KS_\infty \\
G_\infty & e_2 & \Graphs \\};
\draw[->]
 (m-1-3) edge (m-2-3)
 (m-2-1) edge (m-2-2) edge[dashed] (m-1-3)
 (m-2-2) edge (m-2-3);
 \end{tikzpicture}
\]

This is possible since $\KS_\infty\to \Graphs$ is a quasi-isomorphism. See also Appendix \ref{sec:} for lifting up to homotopy.
Using the map $G_\infty \to \KS_\infty$ one can pull back our $KS_\infty$ morphism to a $G_\infty$ morphism
\[
 T_{poly}' \to D_{poly}.
\]
Here the $G_\infty$ structure on the left is not the standard one. We use the prime to distinguish it from the space $T_{poly}$ with the standard Gerstenhaber structure. The homotopy in the above diagram, composed with the representation $\Graphs\to \End(T_{poly})$, gives aus a $G_\infty$ map $T_{poly}\to T_{poly}'$. Composing this map with the above formality morphism finally yields the $G_\infty$ formality morphism
\[
 T_{poly} \to D_{poly}.
\]
Here the Gerstenhaber structure on the left is the usual one, and the $G_\infty$ structure on the right (solution to Deligne's conjecture) comes from pulling back the $KS_\infty$ structure via the lifting map $G_\infty \to \KS_\infty$. 

\begin{lemma}
 Fix a $G_\infty$ structure on $D_{poly}$ given by braces operations only. Assume two $GL(d)$ equivariant $G_\infty$ quasi-isomorphisms $\phi_1, \phi_2: T_{poly}\to D_{poly}$ with the same first order Taylor component are given. Then $\phi_1$ and $\phi_2$ are homotopic.
\end{lemma}
For the proof, pick a homotopy inverse to $\phi_1$, say $\phi_1^{-1}$. It can be chosen in a $GL(d)$ equivariant way by averaging (over $U(n)$). Then the composition $\phi_1^{-1}\circ \phi_2$ is a $G_\infty$ automorphism of $T_{poly}$ and the lemma follows from the following result.

\begin{lemma}
 Any $GL(d)$-equivariant $G_\infty$ automorphism $\phi$ of $T_{poly}$ is homotopic to its first order part $\phi_1$.
\end{lemma}
\begin{proof}
 We give a short proof which is a simple adaptation of the method of \cite{DTT}. Let $\Xi$ be as in that reference. 
We can assume w.l.o.g. that $\phi_1=\mathit{id}$.
It is sufficient to show that the following diagram of Gerstenhaber algebras commutes.
\[
 \begin{tikzpicture}
  \matrix(m)[diagram]{ \Omega_{e_2}(B_{e_2^{\vee}}(T_{poly})) & \Omega_{e_2}(\Xi) & D_{poly} \\};
\draw[->]
 (m-1-1) edge[bend right] node[auto, swap]{$\scriptstyle p$} (m-1-3)
 (m-1-1) edge[bend left] node[auto]{$\scriptstyle p\circ \phi$} (m-1-3)
 (m-1-2) edge (m-1-1)
 (m-1-2) edge (m-1-3);
 \end{tikzpicture}
\]
Here the bottom arrow is the canonical projection and the top arrow is the given automorphism $\phi$, followed by the canonical projection. The leftwards arrow is the inclusion and the remaining arrow is the projection. It is clear that the lower cell commutes. We want to show that the upper cell does so as well. At the end, we need to show that the projection is the only possible $GL(d)$-equivariant Gerstenhaber map $\Omega_{e_2}(\Xi)\to T_{poly}$. Indeed, by degree reasons one can see that the only generators that can be mapped to nonzero values are
\begin{enumerate}
 \item Expressions $u$, for $u$ a function or vector field, which are mapped to $\phi(u)=u$ by assumption.
 \item Expressions $u\wedge v$ for $u,v$ vector fields. By antisymmetry in $u,v$ and by $GL(d)$-equivariance this basis element can only be mapped to $\lambda \dv \co{u}{v}$, for some constant $\lambda$.
 \item Expressions $\underline{fu}$ for $f$ a function and $u$ a vector field. These basis elements can be mapped to $\mu f \dv u + \nu u\cdot f$.
\end{enumerate}
 Similarly to \cite{DTT} one can check that one can set $\lambda=0$ by an appropriate homotopy. Furthermore the condition of being a $G_\infty$-morphism forces $\mu=\nu=\lambda=0$.
\end{proof}

\subsection{On the $L_\infty$ level}
One has the natural embedding of operads $L_\infty\to G_\infty$.
Also, from $Lie\to KS$ one obtains the embedding $\Omega(B(Lie)) \to \KS_\infty$. Precomposing with $L_\infty\to \Omega(B(Lie))$ one obtains a map $L_\infty\to \KS_\infty$, and by postcomposing with the Kontsevich-Soibelman map $L_\infty \to C_\bullet(FM_2)$.

\begin{lemma}
 The maps $L_\infty\to \KS_\infty$ and $L_\infty \to C_\bullet(FM_2)$ are up to homotopy uniquely determined by the image of the binary generator.
\end{lemma}
\begin{proof}
 It follows from degree reasons; there are no classes of appropriate degrees in $H(\KS_\infty)\cong H(FM_2)\cong e_2$.
\end{proof}

In particular, from the lemma it follows that $n$-ary generator is mapped under $L_\infty \to C_\bullet(FM_2)$ to the fundamental chain of $FM_2(n)$, possibly up to (irrelevant) boundaries. A similar argument shows that the $n$-ary part of $hL_\infty\subset \hKS_\infty$ is mapped to the fundamental chain of $D_k(n)$, up to boundaries. From the previous statements it follows that the $L_\infty$ parts of the $KS_\infty$ and the $G_\infty$ formality morphisms agree with Kontsevich's $L_\infty$ morphism \cite{kontsevich}.

